SmartDCA superiority

Dollar-Cost Averaging (DCA) is a widely used technique to mitigate volatility in long-term investments of appreciating assets. However, the inefficiency of DCA arises from fixing the investment amount regardless of market conditions. In this paper, we present a more efficient approach that we name SmartDCA, which consists in adjusting asset purchases based on price levels. The simplicity of SmartDCA allows for rigorous mathematical analysis, enabling us to establish its superiority through the application of Cauchy-Schwartz inequality and Lehmer means. We further extend our analysis to what we refer to as $\rho$-SmartDCA, where the invested amount is raised to the power of $\rho$. We demonstrate that higher values of $\rho$ lead to enhanced performance. However, this approach may result in unbounded investments. To address this concern, we introduce a bounded version of SmartDCA, taking advantage of two novel mean definitions that we name quasi-Lehmer means. The bounded SmartDCA is specifically designed to retain its superiority to DCA. To support our claims, we provide rigorous mathematical proofs and conduct numerical analyses across various scenarios. The performance gain of different SmartDCA alternatives is compared against DCA using data from S\&P500 and Bitcoin. The results consistently demonstrate that all SmartDCA variations yield higher long-term investment returns compared to DCA.

==> sections/old_text.tex <==
\section{Generalized smart DCA}

# Generalization of Smart DCA 

## Introduction

In this article we will generalize the smart DCA to a group of function, that can be all proved to be ordered according to inequalities. So we take the same context as in the previous article

First we will set a fixed base amount $p$ (in USD), such that at times $t_1$ we buy a certain amount of BTC for $p_b$ (USD). Next, at times $t_2$ the amount we buy will depend on the function $F$, of the two prices at both times $p_1$ and $p_2$. As such the total cost is:

$$c=p + p \times F(p_1, p_2)$$

In the previous article we used $F=p_1/p_2$ and we proved the resulting average price is better than the one obtain with the DCA.
Here we go further by choosing a more generalized form $F_n$, with the exponent $n$:

$$F_n(p1, p2)=(p_1/p_2)^n$$

Interestingly, we can observe that for $F_0$ we get back to the DCA, as the exponent of $0$ always gives one, the cost then gives:

$$c=p+p$$

And as a consequence $q=p/p_1 + p/p_2$, and we have the average price:

$$\langle p \rangle = \frac{2p_1p_2}{p_1 + p_2}$$

The **harmonic mean** is thus a special case of a 0 order **adaptive mean**. We conclude that there exist a familly of functions parametrized by $n$ and our primary purpose in this article is to find the structure of such a familly. For ease of notation we are going to refer to the adaptive mean of order $n$ as $\mu_n$. As such we already proved that:

$$\mu_0 \ge \mu_1$$

## Calculating $\mu_n$

From following the same procedure with have the quantity bought of the $nth$ order:

$$q_n=\frac{p}{p_1} + \frac{p}{p_2}\left(\frac{p_1}{p_2}\right)^n$$

And then we simplify:

$$q_n=\frac{p}{p_1} + p\frac{{p_1}^n}{{p_2}^{n+1}}$$

So we obtain the generalize form of the obtained quantity $q_n$:

$$q_n=p \left( \frac{{p_2}^{n+1}+{p_1}^{n+1}}{p_1{p_2}^{n+1}} \right)$$

Implicitly we computed that cost $c_n$:

$$c_n=p + p \left(\frac{p_1}{p_2}\right)^n$$

Then again we can simplify in:

$$c_n= p \left( 1+ \left(\frac{p_1}{p_2}\right)^n\right)$$

And the simplified generalize form is then:

$$c_n= p \left(\frac{p_1^n+p_2^n}{p_2^n}\right)$$

---

Finally we have everything to compute the average price of order $n$, $\mu_n=c_n/q_n$:

$$\LARGE \mu_n = \frac{\cancel{p} \left(\frac{p_1^n+p_2^n}{p_2^n}\right)}{\cancel{p}\left( \frac{{p_2}^{n+1}+{p_1}^{n+1}}{p_1{p_2}^{n+1}} \right)}$$

Wich we can simplify in:

$$\mu_n=\frac{p_1p_2(p_1^n+p_2^n)}{p_1^{n+1}+p_2^{n+1}}$$

And finally we find an equivalent formulation as in the previous article, but for the general case $n$:

$$\mu_n=\frac{(p_2{p_1}^{n+1}+p_1{p_2}^{n+1})}{p_1^{n+1}+p_2^{n+1}}$$


## Inequalities between $n$ and $n-1$ (proof)

Now in the final step, we are going to prove the inequalities for all successive $n=[0, 1, ..., n-1, n]$. Practically what we need to prove is that $\mu_{n-1} \ge \mu_{n}$. If we are able to prove that, then we have found an ordering scheme for all $\mu_n$.

The inequality we need to solves is thus, again we replace $x=p_1$ and $y=p_2$:

$$\frac{\cancel{xy}(x^{n-1}+y^{n-1})}{x^n+y^n} \ge \frac{\cancel{xy}(x^n+y^n)}{x^{n+1}+y^{n+1}}$$

We bring the right numerator on right term to the left term:

$$\frac{x^{n-1}+y^{n-1}}{(x^n+y^n)^2} \ge \frac{1}{x^{n+1}+y^{n+1}}$$

Now we move everything to the left:

$$\frac{(x^{n-1}+y^{n-1})(x^{n+1}+y^{n+1})}{(x^n+y^n)^2} -1 \ge 0$$

The numerator of the inequality can be simplified into: 

$$\frac{(yx^n+xy^n)(x^{n+1}+y^{n+1})}{xy}$$,

So we multiply the inequality by $xy(x^n+y^n)^2$ and we obtain:

$$(yx^n+xy^n)(x^{n+1}+y^{n+1}) - xy(x^n+y^n)^2 \ge 0$$

Finally we distributed everything, $(yx^n+xy^n)(x^{n+1}+y^{n+1})$ gives:

$$yx^{2n+1}+y^{n+2}x^n+x{n+2}y^n+xy^{2n+1}$$

And $xy(x^n+y^n)^2$ gives:

$$yx^{2n+1}+xy^{2n+1}+2x^{n+1}y^{n+1}$$

So we cancel the terms and the inequality reads:

$$y^{n+2}x^n+x^{n+2}y^n-2x^{n+1}+2x^{n+1}y^{n+1} \ge 0$$

Now we factorize by $x^ny^n$ and we obtain the form:

$$x^ny^n(y^2+x^2-2xy) \ge 0$$

Which gives the same polynomial identity as in the previous article:

$$x^ny^n(y-x)^2 \ge 0$$


\section{Point of reference $t=0$}

The most simple point of reference one can choose to compute the smart DCA is times $t=0$.
In the following, we are going to prove that by choosing it, the smart DCA is always better or equal to the DCA. Again at each time step, we choose the base prices $p_b$ upon which the actual cost is computed. Let's compute the total quantity:

\begin{align}
    q=\frac{p_b}{p_0} \left( \frac{1}{p_1^2}\frac{1}{p_2^2}...\frac{1}{p_m^2}\right)\\
    q=\frac{p_b}{p_0}\sum_{i=1}^m \frac{1}{p_i^2}
\end{align}

And now, we compute the cost:
\begin{align}
    c=\frac{p_b}{p_0} \left( \frac{1}{p_1}\frac{1}{p_2}...\frac{1}{p_m} \right)\\
    c=\frac{p_b}{p_0}\sum_{i=1}^m \frac{1}{p_i}
\end{align}

Trivially we can obtain the average price $\langle p \rangle=c/q$:

\begin{align}
    \langle p \rangle=\frac{\sum_{i=1}^m \frac{1}{p_i}}{\sum_{i=1}^m \frac{1}{p_i^2}}
\end{align}

Next, in order to prove the supremacy of the smart DCA, we need to prove the following inequality:

\begin{align}
    \frac{m}{\sum_{i=1}^m \frac{1}{p_i}} \ge \frac{\sum_{i=1}^m \frac{1}{p_i}}{\sum_{i=1}^m \frac{1}{p_i^2}}\\
    m\frac{\sum_{i=1}^m \frac{1}{p_i^2}}{\left(\sum_{i=1}^m \frac{1}{p_i}\right)^2} \ge 1\\
    m\sum_{i=1}^m \frac{1}{p_i^2} \ge \left(\sum_{i=1}^m \frac{1}{p_i}\right)^2 
\end{align}

The last inequality is, in fact, the Cauchy-Schwarz inequality, which we know to be true for all $p_i$ without conditions.


\section{Solving for $m=2$, with initial price $p_0$}

In the previous section, we assumed that $p_0=p_1$, this creates a nice simplification that end-up in a polynomial identity, but this gives a special case and does not take into account the more general case. So in this section, we will consider the case $m=2$, with $p_0\ne p_1$

For ease of notation, we will take the prices $p_0=x$, $p_1=y$, and $p_2=z$. Now by replacing it all in equation (50), we obtain:

\begin{align}
    2 \left( \frac{x}{y^2}+\frac{y}{z^2} \right) \ge \left( \frac{x}{y} + \frac{y}{z}\right) \left( \frac{1}{y} + \frac{1}{z}\right) \\
    2 \left( \frac{xz^2 + y^3}{y^2z^2} \right) \ge \left( \frac{xz+y^2}{yz}\right) \left( \frac{y+z}{yz}\right) \\
    2xz^2+2y^3 \ge (zx+y^2)(y+z)\\
    2xy+2y^3 \ge xyz+xz^2+y^3+y^2z\\
    xz^2+y^2 -xyz -y^2z\ge 0\\
    xz(z-y)+y^2(y-z) \ge 0\\
    xz(z-y)-y^2(z-y) \ge 0\\
    (xz-y^2)(z-y) \ge 0\\
\end{align}

If we get back to the case where $x=y$ then we can trivially show that this equation is true:

\begin{align}
    (yz-y^2)(z-y) \ge 0\\
    y(z-y)^2 \ge 0
\end{align}

However, according to \href{https://www.wolframalpha.com/input?i2d=true&i=%5C%2840%29xz-Power%5By%2C2%5D%5C%2841%29%5C%2840%29z-y%5C%2841%29%E2%89%A50}{wolfram alpha} in the case of $x\ne y$, we have a condition for that inequality to be true: 

\begin{align}
    x>0\\
    y>0\\
    z \ge \frac{y^2}{x}
\end{align}


